Representing Long-term Impact of Residential Building Energy Management using Stochastic Dynamic Programming

Scheduling a residential building short-term to optimize the electricity bill can be difficult with the inclusion of capacity-based grid tariffs. Scheduling the building based on a proposed measured-peak (MP) grid tariff, which is a cost based on the highest peak power over a period, requires the user to consider the impact the current decision-making has in the future. Therefore, the authors propose a mathematical model using stochastic dynamic programming (SDP) that tries to represent the long-term impact of current decision-making. The SDP algorithm calculates non-linear expected future cost curves (EFCC) for the building based on the peak power backwards for each day over a month. The uncertainty in load demand and weather are considered using a discrete Markov chain setup. The model is applied to a case study for a Norwegian building with smart control of flexible loads, and compared against methods where the MP grid tariff is not accurately represented, and where the user has perfect information of the whole month. The results showed that the SDP algorithm performs 0.3 % better than a scenario with no accurate way of presenting future impacts, and performs 3.6 % worse compared to a scenario where the user had perfect information.

==> chapters/temp.tex <==
\makenomenclature

\renewcommand{\nomgroup}[1]{%
\ifthenelse{\equal{#1}{A}{\item[\textbf{SDP sets}]}{%
\ifthenelse{\equal{#1}{B}}{\item[\textbf{Index sets}]}{%
\ifthenelse{\equal{#1}{C}}{\item[\textbf{Parameters}]}{%
\ifthenelse{\equal{#1}{D}}{\item[\textbf{State variables}]}{%
\ifthenelse{\equal{#1}{E}}{\item[\textbf{Stochastic variables}]}{%
\ifthenelse{\equal{#1}{O}}{\item[\textbf{Other}]}{}}}}}}
}

\setlength{\nomlabelwidth}{1.5cm}
\renewcommand\nomgroup[1]{%
  \item[\bfseries
  \ifstrequal{#1}{A}{SDP sets}{%
  \ifstrequal{#1}{B}{Index sets}{%
  \ifstrequal{#1}{C}{Parameters}{%
  \ifstrequal{#1}{E}{Stochastic variables}{%
  \ifstrequal{#1}{D}{Decision variables}{%
  \ifstrequal{#1}{O}{Other Symbols}{}}}}}}%
]}

%For sets
%\nomenclature[A]{$\mathcal{T}_{Stage}$}{set of stages within the period}
\nomenclature[A]{$\mathcal{S}_{t}$}{set of state variables}
\nomenclature[A]{$\mathcal{S}_{s,t}$}{set of stochastic variables}
\nomenclature[A]{$\mathcal{S}_{p,t}$}{set of deciding variables}
%\nomenclature[A]{$\mathcal{N}_{State}$}{List of discrete }
%\nomenclature[A]{$\mathcal{N}_{Scen}$}{set of deciding variables}



\nomenclature[B]{$\mathcal{G}$}{Set of time steps within the stage}


%Stochastic variables
\nomenclature[E]{$\lambda^{Spot}_g$}{Electricity price from spot market in time step g [$\frac{NOK}{kWh}$]}
\nomenclature[E]{$P_{g}^{Inflex}$}{Inflexible load in the household in time step g [$kWh$]}
\nomenclature[E]{$\delta_g^{EV}$}{EV connected to building $\{0,1\}$}
\nomenclature[E]{$I_g^{Irr}$}{Irradiation on PV panels [$\frac{kWh}{m^2}$]}
\nomenclature[E]{$\delta_g^{Occ}$}{Occupancy presence $\{0,1\}$}
\nomenclature[E]{$T^{Out}$}{Daily average outdoor temperature [$\degree C$]}



%Decision variables
\nomenclature[D]{$p_g^{imp}, p_g^{exp}$}{Energy imported/exported to household [$\frac{kWh}{h}$]}
%\nomenclature[D]{$p_g^{exp}$}{Energy exported from household [$\frac{kWh}{h}$]}
\nomenclature[D]{$p^{peak}$}{Peak of imported energy [$\frac{kWh}{h}$]}
\nomenclature[D]{$\gamma$}{SOS-2 variables}

%Special variable
\nomenclature[D]{$C_{p^{peak},s^e_{t+1}}^{peak}$}{Expected future cost from peak power [$\frac{NOK}{\frac{kWh}{h}}$]}

%EV
\nomenclature[D]{$e_g^{soc}$}{State of charge for EV for time step t [$kWh$]}
\nomenclature[D]{$e_g^{ch}$}{Input power to EV for time step t [$\frac{kWh}{h}$]}

%BAT
\nomenclature[D]{$b_g^{soc}$}{State of charge for Battery for time step t [$kWh$]}
\nomenclature[D]{$b_g^{ch},b_t^{dch}$}{Input/output power to battery for time step t [$\frac{kWh}{h}$]}

%PV
\nomenclature[D]{$\theta_g^{prod}$}{Power produced from PV system [$\frac{kWh}{h}$]}

%Heat
\nomenclature[D]{$\mu_g^{indoor}$}{Indoor temperature of the building [$\degree C$]}
\nomenclature[D]{$\mu_g^{Heater}$}{Heater power usage for building heating [$\frac{kWh}{h}$]}
%\nomenclature[D]{$\mu_g^{\Delta T}$}{Change in energy in room [$\frac{kWh}{h}$]}

%Parameters

\nomenclature[C]{$C^{grid}$}{DSO energy tariff for imported energy [$\frac{NOK}{kWh}$]}
\nomenclature[C]{$P^{imp,max}$}{Maximum power import to building [$\frac{kWh}{h}$]}
\nomenclature[C]{$P_n^{Peak}$}{Peak power at point $n$ [$\frac{kWh}{h}$]}
\nomenclature[C]{$P_0^{Peak}$}{Initial peak power [$\frac{kWh}{h}$]}
\nomenclature[C]{$Tax$}{Value added tax for purchase of electricity [$p.u$]}



%EV
\nomenclature[C]{$E^{Cap}$}{EV storage capacity [$kWh$]}
\nomenclature[C]{$\eta^{EV,ch}$}{EV charging efficiency [$\%$]}
\nomenclature[C]{$E^{Max}$}{Maximum EV charging capacity [$kWh$]}
\nomenclature[C]{$E_g^{soc_{min}},E_g^{soc_{max}}$}{Min/Max EV soc capacity [$kWh$]}
\nomenclature[C]{$E^{Load}$}{EV load when not present at home [$kWh$]}
\nomenclature[C]{$E^{Start/Stop}$}{EV start/end soc [$kWh$]}

%HERE I AM, ONCE AGAIN!
%BAT
\nomenclature[C]{$B^{Cap}$}{Battery storage capacity [$kWh$]}
\nomenclature[C]{$\eta^{B,dch},\eta^{B,ch}$}{Discharge/charge efficiency for battery [$\%$]}
\nomenclature[C]{$B^{dch},B^{ch}$}{Discharge/charge capacity for battery [$\frac{kWh}{h}$]}
\nomenclature[C]{$B^{Start/Stop}$}{Battery start/end soc [$kWh$]}
\nomenclature[C]{$B^{Min},B^{Max}$}{Min/Max battery soc capacity [$kWh$]}

%PV
\nomenclature[C]{$A^{roof}$}{PV system area [$m^2$]}
\nomenclature[C]{$\eta^{PV}$}{Total efficiency for PV system [$\%$]}


%Heat
\nomenclature[C]{$M^{Heater}$}{Heater rated capacity [$\frac{kWh}{h}$]}
\nomenclature[C]{$M^{A}$}{Size of building floor area [$m^2$]}
\nomenclature[C]{$M^{T_{Set}}$}{Start/end temperature of the building [$\degree C$]}
\nomenclature[C]{$M_g^{T_{Down}},M_g^{T_{Up}}$}{Lower/upper temperature boundary [$\degree C$]}
\nomenclature[C]{$M^{Storage}$}{specific heat capacity for heating storage in building [$\frac{kWh}{m^2\cdot K}$]}
\nomenclature[C]{$\alpha_g^{HL}$}{Time-dependent heat loss constant [$kWh$]}
\nomenclature[C]{$\beta_g^{HL}$}{Time-dependent heat loss slope [$\frac{kWh}{\degree C}$]}
\nomenclature[C]{$M^{Occ}$}{Heat gained due to occupancy [$\frac{kWh}{h}$]}

\printnomenclature
%For parameters




\begin{align}
    & min \; [Import - Export + Future] \label{eq:Obj_function}\\
    & Import = \sum_{g \in \mathcal{G} } p_g^{imp}\cdot (C^{grid} + \lambda_g^{Spot})\cdot (1+Tax) \nonumber\\
    & Export = \sum_{g \in \mathcal{G} } p_g^{exp}\cdot \lambda_g^{Spot} \nonumber \\
    & Future =  C_{p^{peak},s_{t+1}^{e}}^{peak}   \nonumber
\end{align}
\begin{subequations}
    \begin{flalign}
        & p^{peak} \geq P_0^{Peak} \label{eq:Memory_power}\\
        & p^{peak} \geq p_g^{imp} \quad \forall g\in \mathcal{G} \label{eq:hourly_power}\\
        & C_{p^{peak},s_{t+1}^{e}}^{peak} =   \sum_{n \in \mathcal{N}_{State}} \gamma_n \cdot C_{P_n^{Peak},s_{t+1}^{e}}^{peak} \label{eq:SOS2_decision} \\
        & p^{peak} = \sum_{n \in \mathcal{N}_{State}} \gamma_n \cdot P_n^{Peak} \label{eq:SOS2_binding} \\
        & \sum_{n \in \mathcal{N}_{State}} \gamma_n = 1 \label{eq:SOS2_var}
    \end{flalign}
\end{subequations}
\begin{align}
    & p_g^{imp} - p_g^{exp} + \theta_g^{prod}  + b_g^{dch} = \nonumber \\
    & P_g^{Inflex} + e_g^{ch} + \mu_g^{Heater} + b_g^{ch} \cdot \eta^{B,ch} \quad \forall g \in \mathcal{G} \label{eq:Energy_balance}
\end{align}  
\begin{subequations}
    \begin{align}
    & e_g^{soc}-e_{g-1}^{soc} = e_g^{ch}\eta^{EV,ch}(\delta_g^{EV}) \nonumber \\
    & -E^{Load} (1-\delta_g^{EV}) \quad  \forall g \in \mathcal{G} \backslash g \neq 1 \label{eq:EV_soc_balance} \\
    & e_g^{soc} - E^{Start/Stop} = \nonumber \\
    & e_g^{ch} \eta^{EV,ch}-E^{Load}\cdot (1-\delta_g^{EV}) \quad g = 1 \label{eq:soc_balance_EV} \\
    & E^{Start/Stop} = e_g^{soc} \quad g = 24 \label{eq:soc_balance,init} \\
    & 0 \leq e_g^{ch} \leq E^{Max} \quad \forall g \in \mathcal{G} \label{eq:EV_charge_lim} \\
    & E_g^{soc,min} \leq e_g^{soc} \leq E_g^{soc,max} \quad \forall g \in \mathcal{G} \label{eq:EV_soc_lim} 
    \end{align}
\end{subequations}

\begin{subequations}
    \begin{align}
    & b_g^{soc} - b_{g-1}^{soc} = b_g^{ch} - \frac{b_g^{dch}}{\eta^{B,dch}} \quad \forall g \in \mathcal{G} \backslash g \neq 1 \label{eq:BAT_balance} \\
    & b_g^{soc} - B^{{Start/Stop}} = b_g^{ch} - \frac{b_g^{dch}}{\eta^{B,dch}} \quad g = 1 \label{eq:BAT_balance_init} \\
    & b_g^{soc} = B^{{Start/Stop}}  \quad g = 24 \label{eq:BAT_balance_end} \\
    & 0 \leq b_g^{ch} \leq B^{ch,max} \quad \forall g \in \mathcal{G} \label{eq:Bat_charge_lim} \\
    & 0 \leq b_g^{dch} \leq B^{dch,max} \quad \forall g \in \mathcal{G} \label{eq:Bat_discharge_lim} \\
    & B^{Min} \leq b_g^{soc} \leq B^{Max} \quad \forall g \in \mathcal{G} \label{eq:Bat_soc_lim} \\
    \end{align}
\end{subequations}

\begin{align}
    & \theta_g^{prod} = A^{roof} \cdot \eta^{PV}\cdot I_g^{Irr} \quad \forall g \in \mathcal{G} \label{eq:PV_prod} 
\end{align}

\begin{subequations}
    \begin{align}
    & \mu_g^{Heater} + M^{Occ}\cdot \delta_g^{Occ} = \mu_g^{\Delta T} + M^{HL}_g \quad \forall g \in \mathcal{G} \label{eq:Heat_balance} \\ 
    & \mu_g^{\Delta T} = M^{A} M^{soc} (\mu_g^{indoor} - \mu_{g-1}^{indoor}) \; \forall g \in \mathcal{G} \backslash g \neq 1 \\
    & \mu_g^{\Delta T} = M^{A} M^{soc} (\mu_g^{indoor} - M^{T_{Set}}) \quad g = 1 \\
    & \mu_g^{indoor} = M^{T_{Set}} \quad g = 24 \label{eq:Heat_balance_end} \\
    & M^{HL}_t = \alpha_g^{HL} + \beta_g^{HL}\cdot T^{Out}  \quad \forall g \in \mathcal{G} \label{eq:HL} \\
    & 0 \leq \mu_g^{Heater} \leq M^{Rated} \quad \forall g \in \mathcal{G} \label{eq:Heater} \\
    & M_g^{T_{Down}} \leq \mu_g^{indoor} \leq M_g^{T_{Up}} \quad \forall g \in \mathcal{G} \label{eq:Heat_lim_empty}
    \end{align}
    \label{eq:heat}
\end{subequations}


The second suggested tariff, measured peak, is on the contrary to subscribed capacity straightforward to implement (with smart meters) and exists for many commercial/industrial customers today. It is fairly understandable, also for passive end-users, and capacity is priced directly without any action required on forehand. Costs are also fairly predictable, which translates to stable incomes for the DSOs. However, there are significant drawbacks of this tariff. With costs being based on monthly peaks, a very high peak early in the month removes all incentives to reduce peaks for the rest of the month. Therefore, peaks can be hard to predict and can happen somewhat randomly. Thus, a methodology to predict peaks and plan for it is required. Advantages and drawbacks of both the two grid tariff structures are presented in \Cref{tariffadvantages}.

\begin{table}[h]

\begin{tabular}{lcc}
                                        & \multicolumn{1}{l}{\textbf{Measured peak}}                                                                         & \multicolumn{1}{l}{\textbf{Subscribed capacity}}                                                  \\ \hline
\multicolumn{1}{c}{\textbf{Advantages}} & \begin{tabular}[c]{@{}c@{}}1) Easy to implement\\ 2) Easy to understand\\ 3) Predictable costs\end{tabular}           & \begin{tabular}[c]{@{}c@{}}1) Predictable costs\\ 2) Incentivizes\\ active customers\end{tabular} \\ \hline
\textbf{Drawbacks}                      & \begin{tabular}[c]{@{}c@{}}1) Early peaks removes\\ peak shaving incentives\\ 2) Hard to predict peak\end{tabular} & \begin{tabular}[c]{@{}c@{}}1) Hard to implement\\ 2) Hard to understand\end{tabular}              \\ \hline
\end{tabular}
\caption{Advantages and drawbacks of measured peak and subscribed capacity grid tariff structures.}
\label{tariffadvantages}
\end{table}


\newpage
hello
\newpage

\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}



Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,references}


\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.

